Improving Fast Minimum-Norm Attacks with Hyperparameter Optimization

Evaluating the adversarial robustness of machine learning models using gradient-based attacks is challenging. In this work, we show that hyperparameter optimization can improve fast minimum-norm attacks by automating the selection of the loss function, the optimizer and the step-size scheduler, along with the corresponding hyperparameters. Our extensive evaluation involving several robust models demonstrates the improved efficacy of fast minimum-norm attacks when hyper-up with hyperparameter optimization. We release our open-source code at https://github.com/pralab/HO-FMN.

==> ray_fmn_framework.tex <==
The Ray Tune Framework \cite{liaw2018tune} can be summarized as a block scheme in which it is necessary to specify: \textit{(i)} a \textbf{search space} which defines ranges and sampling of the hyperparameter values; \textit{(ii)} a \textbf{trainable} which defines the objective to be optimized; \textit{(iii)} a \textbf{search algorithm} and a \textbf{scheduler}, which respectively suggests the hyperparameter configurations (for instance a grid search) and optimizes the search by deciding when and where to stop within the hyperparameters' search space. 
The output of the Ray Tune framework is a set of generated trials which are chosen by the scheduler-search algorithm pair and executed. A trial \cite{liaw2018tune}, can be defined as a single run with a fixed initial hyperparameter configuration where, however, the hyperparameters configuration can be tweaked on-the-fly and/or early stopped in favor of others.

\begin{figure}[h!]
\centering
\includegraphics[width=0.8\textwidth]{images/FmnOpt.png}
\caption{Ray Tune framework adapted for the FMN Hyperparameter Optimization.}\label{Fig:fmn_opt}
\end{figure}

In this work, we embed our FMN hyperparameter optimization problem into the Ray Tune framework, as shown in \autoref{Fig:fmn_opt}. The search space in our application scenario, is represented by the set of optimizers and step-size schedulers. The losses, being only two, have instead been chosen not to be part of the search space and rather be selected manually to create 2x configurations. 
The trainable objective, is represented by the FMN attack applied on a pool of robust models available on the standardized robustness benchmark RobustBench \cite{croce20-robustbench} (the models are listed in Section~\ref{sect:exp}). The search algorithm CFO \cite{wu2020AAAI-cfo} and the ASHA scheduler \cite{li2020-asha} have been instead chosen as algorithms responsible for finding the best optimizer and step-size scheduler for the attack. Through the proposed framework, we gather a set of best optimizer/scheduler/loss configurations for the various robust models. Additionally, for each model, we run the FMN attack with its best configuration and study the robustness evaluation results we get from such adaptation of the FMN configuration to every specific model studied.



